LYRA I: Simulating the multi-phase ISM of a dwarf galaxy with variable energy supernovae from individual stars

We introduce the LYRA project, a new high resolution galaxy formation model built within the framework of the cosmological hydro-dynamical moving mesh code AREPO. The model resolves the multi-phase interstellar medium down to 10 K. It forms individual stars sampled from the initial mass function (IMF), and tracks their lifetimes and death pathways individually. Single supernova (SN) blast waves with variable energy are followed within the hydrodynamic calculation to interact with the surrounding interstellar medium (ISM). In this paper, we present the methods and apply the model to a $10^{10} M_{\odot}$ isolated halo. We demonstrate that the majority of supernovae are Sedov-resolved at our fiducial gas mass resolution of $4 M_{\odot}$. We show that our SN feedback prescription self-consistently produces a hot phase within the ISM that drives significant outflows, reduces the gas density and suppresses star formation. Clustered SN play a major role in enhancing the effectiveness of feedback, because the majority of explosions occur in low density material. Accounting for variable SN energy allows the feedback to respond directly to stellar evolution. We show that the ISM is sensitive to the spatially distributed energy deposition. It strongly affects the outflow behaviour, reducing the mass loading by a factor of 2-3, thus allowing the galaxy to retain a higher fraction of mass and metals. LYRA makes it possible to use a comprehensive multi-physics ISM model directly in cosmological (zoom) simulations of dwarf and higher mass galaxies.

==> cosmo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INTRO ideas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dwarfs:
% building blocks of galaxy formation in hierarchical picture
% most numerous type of galaxy
% low metallicity systems (Tremonti et al. 2004; Hunter et al. 2012)
% ideal laboratories for studying physical processes of the ISM under chemically simple conditions

% Feedback:
% indispensable ingredient in the theory of galaxy formation and evolution (Larson 1974; White & Rees 1978; Dekel & Silk 1986; Mac Low & Ferrara 1999)
% with feedback, observed properties can be recovered (Somerville & Dave ́ 2015 and Naab & Ostriker 2017 and references therein)
% most of them have to resort to ad hoc sub-grid recipes in order to make the feedback efficient due to resolution
% should be viewed as a phenomenological ‘input’ of the model
% cannot investigate how feedback couples to the gas dynamics on parsec scales

% Small scale sims:
% trade-off: focus only on a single gas cloud or a small patch of a galaxy (see e.g. Joung & Mac Low 2006; Dale & Bonnell 2011; Kim, Kim & Ostriker 2011; Hill et al. 2012; Walch et al. 2012, 2015; Simpson et al. 2016; Naab & Ostriker 2017)

% dwarf galaxy sims:
% (Kim et al. 2013a,b; Forbes et al. 2016; Hu et al. 2016)

% Lower res cosmo sims:
% chemodynamical evolution of galaxies using cosmological hydrodynamics simulations (e.g. Oppenheimer & Dave ́ 2008; Wiersma et al. 2009; Shen, Wadsley &Stinson 2010; Simpson et al. 2013; Snaith et al. 2015; Schaye et al. 2010, 2015; Hopkins et al. 2014)
% remarkable progress in reproducing global galaxy trends such as evolution of the mass–metallicity relationship (e.g. Obreja et al. 2014; Ma et al.2016a;Dave ́ et al. 2017;Torrey et al. 2017)
% Another aspect of the modelling of baryons in simulations that is under debate is how to accurately follow the supernova shocks themselves. Only sufficiently high mass and spatial resolution can resolve the Sedov phase and self-consistently drive flows through the ISM and out of galaxies. With less resolution, a purely thermal injection of a supernova is unresolved and the energy is quickly radiated away before it is turned into momentum \citep[e.g.][]{DallaVecchia2008}.

%Keller
% Supernovae  (SNe)  are  important  components  of  any  theory  of galaxy  formation,  in  both  (semi-)analytic  models  and  hydrodynamic  simulations.  The  energy  and  momentum  injected  by  SNe stirs  turbulence  in  the  interstellar  medium  (ISM)  (Joung  &  MacLow 2006), drives the formation of a multiphase ISM (McKee &Ostriker  1977),  and  can  launch  galaxy-scale  winds  and  outflows(Larson 1974). Modelling SNe in galaxy formation simulations has proven to be non-trivial. The failure of SNe to regulate star formation in early simulations (Katz 1992; Scannapieco et al. 2012) hasled to significant effort to develop sub-grid treatments of SNe insimulations where the early, small-scale evolution of SN remnantsare unresolved (Thacker & Couchman 2000; Springel & Hernquist2003; Stinson et al. 2006; Dalla Vecchia & Schaye 2012; Kelleret al. 2014).

%Hu
% indispensable ingredient in the theory of galaxy formation and evolution \citep{Larson1974, Saito1979, White1978, Dekel1986, Mac Low & Ferrara 1999)
% with feedback, observed properties can be recovered (Somerville & Dave ́ 2015 and Naab & Ostriker 2017 and references therein)
% most of them have to resort to ad hoc sub-grid recipes in order to make the feedback efficient due to resolution
% should be viewed as a phenomenological ‘input’ of the model
% cannot investigate how feedback couples to the gas dynamics on parsec scales


% It seems that increased resolution is necessary to better understand the feedback process, but computational constraints still prevent this level of resolution in massive galaxies. So simulating dwarf galaxies has become the weapon of choice. However, there are other reasons for choosing to investigate dwarf galaxy evolution. For one, dwarfs have a low enough SFR that it is easier to disentangle the effects of various feedback processes happening simultaneously. Additionally, these small halos represent the edge of galaxy formation. Understanding in which environment star formation can proceed and below which mass halos remain dark can give important clues to the SF process and baryonic feedback. Since the potential wells of dwarf galaxies are extremely shallow, reionization can easily quench them. But the shallow potential well can also be more sensitive to baryonic processes altering its shape, making these systems great targets for answering the cusp-core question \citep{cusp-core}. Field dwarfs are also assumed to be the progenitors of satellite galaxies that enter the halos of larger galaxies such as the Milky Way. So understanding their properties before in fall can give vital clues to the effects of ram pressure stripping and satellite quenching \citep{satellites}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% As most state-of-the-art cosmological simulations to date, the
% equations of motion are integrated into a Friedman-Robertson-Walker
% metric for which we use the latest cosmological parameters published by
% the \citet{PlanckCollaboration2014}. 
%
% \subsection{Cosmological dwarf galaxy}
% \label{sec:cosmo}
% %==========================================================================%
% %
% Ongoing SF after reionization:
% One startling aspect of dwarf galaxies is that there seem to be a category of faint dwarf galaxies with ongoing star formation at $z=0$, such as Leo T, Leo A and Leo P \citep{Cole2007, Cole2014, Weisz2014}. 
% Some proposed reasons for intermittent and late-time ongoing SF in simulations are:
% equal-mass mergers \citep{Benitez-Llambay2016}
% gaining enough halo mass \citep{Benitez-Llambay2015, Fitts2017, Ledinauskas2018}
% interactions with IGM gas causing gas compression \citep{Wright2019}
%
% From observations:
% SF burst after increase in concentration \citep{Ricotti2009}
% inefficient and slow gas cooling \citep{Cole2014}
%
% We put our model to the test with a cosmological zoom simulation of an $5\times10^9\Msun$ halo mass dwarf galaxy. The initial conditions were created by \citet{Jenkins2013} and are derived from the EAGLE \citet{Schaye2015} box. The $\Lambda$CDM cosmological parameters are $\Omega_{\Lambda} = 0.693$, $\Omega_0 = 0.307$, $\Omega_b = 0.048$ and $h=0.6777$. The full box is $100$Mpc/h and includes three zoom levels. The dark matter mass is $L\approx 770\Msun$ with $\varepsilon_{\rm dm}=10$pc gravitational softening that is fixed at its physical value from $z=10-0$. We set the target gas mass to $4\Msun$ with a gravitational softening of $\varepsilon_{\rm gas}=0.5$pc. The stellar particles share the same softening as the gas. 

% We now turn to presenting the stellar and hydrodynamic properties of our simulation. We compare to observation where appropriate and attempt to determine how similar our simulated dwarf galaxy is to known dwarf galaxies.

% First, we show the star formation history (SFH) in fig. \ref{fig:SFH}. 
% \begin{figure}
%   \includegraphics[width=\linewidth]{images/{SFH_0.5Gyr}.pdf}
%   \caption[]{SFH in bins of $0.5$\,Gyr.}
%   \label{fig:SFH}
% \end{figure}
% %
% \begin{figure}
%   \includegraphics[width=\linewidth]{images/SMHM.pdf}
%   \caption[]{Stellar mass to halo mass relation with the $z=0$ value for our cosmological simulation.}
%   \label{fig:SMHM}
% \end{figure}
% %
% \begin{figure}
%   \includegraphics[width=\linewidth]{images/size-mass_relation.pdf}
%   \caption[]{Size - mass relation showing observational data from the compilation of \citet{Misgeld13}. }
%   \label{fig:size-mass}
% \end{figure}
% %
% \begin{figure}
%   \includegraphics[width=\linewidth]{images/stellar-mass-metallicity.pdf}
%   \caption[]{Stellar mass - metallicity relation with the $z=0$ value for our cosmological simulation. Observational data are from \citet{Kirby13} showing Local Group and Andromeda dwarf galaxies.}
%   \label{fig:mass-metallicty}
% \end{figure}
%
